A Lightweight Blockchain and Fog-enabled Secure Remote Patient Monitoring System

IoT has enabled the rapid growth of smart remote healthcare applications. These IoT-based remote healthcare applications deliver fast and preventive medical services to patients at risk or with chronic diseases. However, ensuring data security and patient privacy while exchanging sensitive medical data among medical IoT devices is still a significant concern in remote healthcare applications. Altered or corrupted medical data may cause wrong treatment and create grave health issues for patients. Moreover, current remote medical applications' efficiency and response time need to be addressed and improved. Considering the need for secure and efficient patient care, this paper proposes a lightweight Blockchain-based and Fog-enabled remote patient monitoring system that provides a high level of security and efficient response time. Simulation results and security analysis show that the proposed lightweight blockchain architecture fits the resource-constrained IoT devices well and is secure against attacks. Moreover, the augmentation of Fog computing improved the responsiveness of the remote patient monitoring system by 40%.

==> table.tex <==
\begin{scriptsize}
\begin{table}
\label{tab:summ}
\caption{Summary of related works}
\small
\resizebox{1.1\textwidth}{!}{%
\begin{tabular}{|p {1.5 cm}|p {3cm}|p {1.8 cm}|p {1.5 cm}|p {2 cm}|p {1.5 cm}|p {2 cm}|p {2 cm}|p {2 cm}|p {2 cm}|}
\hline 
Ref & Contribution/ Purpose & Blockchain Type & Framework & Consensus&Data Type & Storage & Validation Tools & Merits & Limits \\ 
\hline 
\cite{griggs2018healthcare} & Sharing healthcare data for clinical and research purposes. & Private/ Consortium &Ethereum &PBFT & IoMT & ... & Solidity + Smart contracts& • & Sensors data are sent regularly to the patient phone, which will consume its energy and make solution not practical and dependent on the user phone\\ 
\hline 
... &  . &... &Ethereum &PBFT & IoMT & ... & Solidity + Smart contracts& • &  \\ 
\hline 

MedBlock: \cite{fan2018medblock} & Sharing healthcare data for clinical and research purposes. & Public &N/A & An endorser is elected by more than half of the nodes. Then, the endorser validate transactions.& EHR & Local Database & Security analysis.  Latency of service provider requests& • & The endorser is a central entity which minimizes the advantages of the distributed nature of blockchain. No implementation is done \\ 
\hline 
MedChain: \cite{shen2019medchain} & Healthcare Data Sharing &Consortium blockchain  & Java & BFT-SMaRt \cite{sousa2012byzantine} & EHR + IoMT & Local Database & Implementing using Java& &The frequent intervention of healthcare providers is needed. \\ 
\hline 

\cite{attia2019iot} &Remote Patient  Monitoring& Private &Hyperledger Fabric &... & IoMT & ... & .& • &  \\ 
\hline 
\cite{jabbar2020blockchain} &Remote Patient  Monitoring& Private &Hyperledger Fabric &... & IoMT & ... & .& • &  \\ 
\hline 

 \cite{khatoon2020blockchain} & Design and implementation of different medical workflows &Private  & Ethereum &PoW (Ethash)& EHR  & Back-end distributed file system (DFS) & solidity language+ Remix and Kovan test network& & Only partial system is developed\\ 
\hline
\cite{jamil2020towards} & Vital signs real time remote monitoring &Private  & Hyperledger Fabric &PoW& IoMT  & Distributed
ledger technology (DLT) & Hyperledger Fabric + Caliper& &The storage of patients data in blockchain network is a heavy. \\ 
\hline 
\end{tabular} }
\end{table}
\end{scriptsize}
